A Survey on Video Diffusion Models

The recent wave of AI-generated content (AIGC) has witnessed substantial success in computer vision, with the diffusion model playing a crucial role in this achievement. Due to their impressive generative capabilities, diffusion models are gradually superseding methods based on GANs and auto-regressive Transformers, demonstrating exceptional performance not only in image generation and editing, but also in the realm of video-related research. However, existing surveys mainly focus on diffusion models in the context of image generation, with few up-to-date reviews on their application in the video domain. To address this gap, this paper presents a comprehensive review of video diffusion models in the AIGC era. Specifically, we begin with a concise introduction to the fundamentals and evolution of diffusion models. Subsequently, we present an overview of research on diffusion models in the video domain, categorizing the work into three key areas: video generation, video editing, and other video understanding tasks. We conduct a thorough review of the literature in these three key areas, including further categorization and practical contributions in the field. Finally, we discuss the challenges faced by research in this domain and outline potential future developmental trends. A comprehensive list of video diffusion models studied in this survey is available at https://github.com/ChenHsing/Awesome-Video-Diffusion-Models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> tex/editing.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\tiny,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=1em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4em,font=\tiny,}{},
            where level=2{text width=3.5em,font=\tiny,}{},
            [
                Video Editing, ver
                [
                    Text-guided
                    % \\ (\S \ref{sec:mcot_bridge})
                    [
                        Training-based
                        [
                            GEN-1~\cite{gen1}{, } Dreamix~\cite{dreamix}
                            , leaf, text width=6.0em
                        ]
                    ]
                    [
                        Training-free
                        [
                            TokenFlow~\cite{geyer2023tokenflow}{, } VidEdit~\cite{couairon2023videdit}{, } Render-A-Video~\cite{yang2023rerenderavideo}{,} \\ Vid2Vid-Zero~\cite{vid2vid-zero}{,} FateZero~\cite{qi2023fatezero}{,} Pix2Video~\cite{ceylan2023pix2video}
                            {,} \\
                            InFusion~\cite{infusion}{,} ControlVideo~\cite{controlvideo}
                            , leaf, text width=11.5em
                        ]
                    ]
                    [
                        One-shot-tuned
                        [
                            SAVE~\cite{save}{,} EI$^2$~\cite{ei2}{,}
                            Edit-A-Video~\cite{shin2023editavideo}{, } Tune-A-Video~\cite{tuneavideo}{, }\\ Video-P2P~\cite{liu2023videop2p}{,} ControlVideo~\cite{controlvideoone-shot}{,} Shape-aware TLVE~\cite{satlve}
                            , leaf, text width=13.5em
                        ]
                    ]
                ]
                [
                    Modality-guided
                    % \\ (\S \ref{sec:mcot_learn})
                    [
                        Instruct-guided
                        [
                           Instruct-vid2vid\cite{qin2023instructvid2vid}{,} CSD~\cite{CSD}
                            , leaf, text width=7.5em
                        ]
                    ]
                    [
                        Sound-Guided
                        [
                            Soundini~\cite{lee2023soundini}{,} SDVE~\cite{sdve}
                            , leaf, text width=5.5em
                        ]
                    ]
                    [
                        Motion-Guided
                        [
                            VideoControlNet~\cite{videocontrolnet}
                            , leaf, text width=4.5em
                        ]
                    ]
                    [
                        Multi-Modal
                        [
                            Make-A-Protagonist~\cite{zhao2023makeaprotagonist} {,} DiffusionVideoEditing~\cite{DiffusionVideoEditing}
                            , leaf, text width=11.5em
                        ]
                    ]
                ]
                [
                    Domain-specific
                    [
                        Video Recolor
                        [
                            ColorDiffuser~\cite{colorDiffusers}
                            , leaf, text width=4.5em
                        ]
                    ]
                    [
                        Video Restyle
                        [
                            Style-A-Video~\cite{styleavideo}
                            , leaf, text width=4.5em
                        ]
                    ]
                    [
                        Human Video
                        [
                            Diffusion Video Autoencoders~\cite{diffusionvideoautoencoder}{,} Instruct-Video2Avatar~\cite{instruct-video2avatar}
                            , leaf, text width=13em
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of Video Editing. Key aspects of Video Editing include General Text-guided Video Editing, Modality-guided Video Editing  and Domain-specific Video Editing. }
    \label{taxo_of_mcot}
\end{figure*}



==> tex/tab_edit.tex <==
\begin{table*}[]
\scalebox{0.83}{
\begin{tabular}{rllll}
\hline
Method  & Year & Datasets & Task                     & Highlight \\ \hline
GEN-1~\cite{gen1}   & 2022 & \cite{davis}    & Text-conditioned & \begin{tabular}[c]{@{}l@{}}GEN-1 shows for the first time that jointly training on image and video data enables \\ inference-time control over temporal consistency.    \end{tabular} \\
Dreamix~\cite{dreamix} & 2023 & - & Text-conditioned & Dreamix is the first text-based appearance and motion editing of real-world videos.          \\
TokenFlow~\cite{geyer2023tokenflow} & 2023 & \cite{davis}  & Text-conditioned & TokenFlow can work with any pre-trained T2I method and has increased temporal consistency. \\
TCVE~\cite{TCVE} & 2023 & \cite{tuneavideo} & Text-conditioned & TCVE enables temporal-consistent video editing. \\
Control-A-Video~\cite{Control-A-Video} & 2023 & \cite{laion400m} & Text-conditioned & \begin{tabular}[c]{@{}l@{}}Control-A-Video can generate arbitrary-length auto-regressively by leveraging first-frame \\ conditioning strategy.    \end{tabular}   \\
VidEdit~\cite{couairon2023videdit} & 2023 & \cite{davis} & Text-conditioned  & VidEdit has huge advantage in terms of foreground and background object editions.   \\
Vid2Vid-Zero~\cite{vid2vid-zero} & 2023 & - & Text-conditioned & Vid2Vid-Zero is the first zero-shot video editing framework directly uses T2I model.      \\
FateZero~\cite{qi2023fatezero} & 2023 & - & Text-conditioned & FateZero is the first zero-shot text-based video editing framework based on T2I model.           \\
Pix2Video~\cite{ceylan2023pix2video} & 2023 & \cite{davis} & Text-conditioned & Pix2Video does not require any pre-processing and does not incur any additional overhead.  \\
InFusion~\cite{infusion} & 2023 & \cite{davis} & Text-conditioned & InFusion enables zero-shot complex concept video editing.   \\
ControlVideo$_\text{1}$~\cite{controlvideo} & 2023 & \cite{davis} & Text-conditioned &  ControlVideo is highly efficient in generating both short and long videos.   \\
EVE~\cite{EVE} & 2023 & \cite{davis, EVE} & Text-conditioned & EVE constructs the ZVE-50 video editing dataset as a novel benchmark for fair comparisons. \\
MeDM~\cite{MeDM} & 2023 & - & Text-conditioned & MeDM requires no video data finetuing or test time optimization. \\
SAVE~\cite{save} & 2023 & \cite{davis} & Text-conditioned & SAVE reduces the editing time significantly.    \\
EI$^2$~\cite{ei2} & 2023 & - & Text-conditioned & EI$^2$ reveals that new parameters cause semantic inconsistency and provides an effective solution. \\
Edit-A-Video~\cite{shin2023editavideo} & 2023 & - & Text-conditioned & Edit-A-Video is the first one-shot video editing framework uses T2I model.   \\
Tune-A-Video~\cite{tuneavideo} & 2023 & \cite{davis} & Text-conditioned & Tune-A-Video is the first T2V generation work using pre-trained T2I models.   \\
Video-P2P~\cite{liu2023videop2p} & 2023 & - & Text-conditioned & Video-P2P is the first framework for video editing with attention control.  \\
ControlVideo$_\text{2}$~\cite{controlvideoone-shot} & 2023 & \cite{davis} & Text-conditioned &  ControlVideo achieves high realism and fidelity while still aligning with the textual prompt.   \\
Shape-aware TLVE~\cite{satlve} & 2023 & \cite{davis} & Text-conditioned & Shape-aware TLVE presents a deformation formulation to handle target shape edits.\\
SinFusion~\cite{Sinfusion} & 2023 &          & Text-conditioned & SinFusion is the first diffusion model trained on a single image/video.   \\
StableVideo~\cite{chai2023stablevideo} & 2023 & \cite{davis} & Text-conditioned & StableVideo is the first to leverage layered atlas to solve consistency problems. \\
Instruct-vid2vid~\cite{qin2023instructvid2vid} & 2023 & \cite{qin2023instructvid2vid} & Modality guided & Instruct-vid2vid is the first training-free end-to-end instruction-guided video editing work.          \\
CSD~\cite{CSD} & 2023 & \cite{davis} & Modality guided & CSD strikes a balance between source-target consistency and instruction fidelity. \\
SDVE~\cite{sdve} & 2023 & \cite{GRID, crema} & Modality guided & SDVE is the first end-to-end audio-driven video editing work.          \\
Soundini~\cite{lee2023soundini} & 2023 & \cite{davis} &  Modality guided  & \begin{tabular}[c]{@{}l@{}}Soundini can synthesize a visual effect that reflects properties of sound (\emph{e.g.} temporal context, \\ intensity, volume).    \end{tabular}   \\
VideoControlNet~\cite{videocontrolnet} & 2023 & \cite{davis, HEVC, uvg, mcl-jcv} & Modality guided & VideoControlNet is a novel video-to-video translation framework inspired by video coding.   \\
Make-A-Protagoist~\cite{zhao2023makeaprotagonist} & 2023 & - & Modality guided & Make-A-Protagonist is the first generic video editing with both visual and textual clues.\\
DragNUWA~\cite{DragNUWAFC} & 2023 & \cite{webvid}, VideoHD & Modality guided & DragNUWA integrates text, image and trajectory controls to generate satisfactory videos.  \\
ColorDiffuser~\cite{colorDiffusers} & 2023 & \cite{webvid} & Domain-specific & \begin{tabular}[c]{@{}l@{}}ColorDiffuser can colorize monochrome videos with diverse and consistent colors through \\ multiple frames based on optional textual descriptions.   \end{tabular}\\
DVAE~\cite{diffusionvideoautoencoder} & 2023 & \cite{voxceleb}  & Domain-specific & DVAE can satisfy both reconstruction and edit capabilities at the same time. \\
Instruct-Video2Avatar~\cite{instruct-video2avatar} & 2023 & - & Domain-specific        & \begin{tabular}[c]{@{}l@{}}Instruct-Video2Avatar can be extended to the editing of arbitrarily static or dynamic NeRFs, \\ even for arbitrary video editing.      \end{tabular}       \\
TGDM~\cite{tgdm} & 2023 & \cite{voxceleb, mead, CelebAMask-HQ} & Domain-specific & TGDM preserves explicit structural information but avoids complex texture deformations.         \\
\hline
\end{tabular}
}
\caption{Representative works summarization and comparison in Sec~\ref{Sec:videoediting}. We list the published year, datasets, involved task and highlighted features here. }
\end{table*}

==> tex/tab_t2v.tex <==
\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}rrccl@{}}
\toprule
Method       & Year & Backbone         & Training Data                                                     & Highlight                                                                                 \\ \hline
\rowcolor{gray!25}  \multicolumn{5}{c}{\bf Non-diffusion based method}                                                                                                                                                         \\ \hline
GODIVA~\cite{wu2021godiva}       & 2021     &   -               &  Howto100M~\cite{howto100m}                                                                 & GODIVA is the first to use VQ-VAE for open-wild T2V task.                                                                                          \\
CogVideo~\cite{hong2022cogvideo}     & 2022     &    CogView2~\cite{ding2022cogview2}              &  WebVid-5.4M~\cite{webvid}                                                                 &  CogVideo is the first open-sourced pretrained Transformer for general T2V task.                                                                                         \\
PHENAKI~\cite{villegas2022phenaki}     & 2022     &  ViViT~\cite{vivit}                & 15M*                                                                  & PHENAKI can generate videos from time vaiable prompts with few tokens computing.                                                                                          \\
NUWA~\cite{wu2022nuwa}         & 2022     &   -               &  VATEX-241K~\cite{vatex}                                                                 & NUWA is an unified multimodal generation methods, covering language, image and video synthesis.                                                                                          \\
MMVG~\cite{mmvg}         & 2023     &   -               &   WebVid-2.5M~\cite{webvid}                                                                & MMVG proposes a uni-model for text guided video prediction, infilling and generation.                                                                                          \\
 \hline
\rowcolor{gray!25} \multicolumn{5}{c}{\bf Diffusion based method}                                                                                                                                                             \\ \hline

Text2Video-Zero~\cite{Text2video-zero}    &2023       & LDM~\cite{stablediffusion}    & Training-free   &  Text2Video-Zero is the first work exploring training-free method for T2V task. \\

DirecT2V~\cite{DirecT2V}    &2023       & LDM~\cite{stablediffusion}    & Training-free   & DirecT2V applies large language models to produce detail caption for training-free T2V model. \\
Free-bloom~\cite{freebloom}    &2023       & LDM~\cite{stablediffusion}    & Training-free   & Free-Bloom propose several modification in reverse
process to generate consistence video. \\
\midrule

VDM~\cite{vdm}          & 2022 &  -                & WebVid-10M~\cite{webvid}                                                                   & VDM is the first video diffusion model to explore large-scale T2V tasks.   \\ 
Make-A-Video~\cite{singer2022make}          & 2022 & DALLE-2~\cite{dalle2}                 &  \begin{tabular}[c]{@{}l@{}}HD-VILA-10M~\cite{hd-vila}+\\ WebVid-10M~\cite{webvid}\end{tabular}                                                                 &
\begin{tabular}[c]{@{}l@{}}Make-A-Video is the first to  explore how to train a T2V model using a large-scale datasets of \\   image-text pairs and unlabeled videos.\end{tabular}    
                  \\ 
Imagen Video~\cite{ho2022imagenvideo}          & 2022 &  Imagen~\cite{imagen}                &   14M*                                                                &\begin{tabular}[c]{@{}l@{}}Imagen Video validates the effectiveness of many training methods in T2I tasks, while also utilizing \\ progressive distillation to accelerate the sampling time of the video diffusion model.    \end{tabular} 
                                                                                       \\ 
MagicVideo~\cite{magicvideo}   & 2022 & LDM\cite{stablediffusion} & \begin{tabular}[c]{@{}l@{}}HD-VILA-10M~\cite{hd-vila}+\\ WebVid-10M~\cite{webvid}\end{tabular} & MagicVideo focuses on improving the data and computational efficiency of video generation model. \\
LVDM~\cite{lvdm}          & 2022 & LDM~\cite{stablediffusion}                 & WebVid-2M~\cite{webvid}                                                                  & LVDM utilizes mask sampling to generate longer videos (one thousand frames) beyond the training length.                                                                                          \\ 

VideoFusion~\cite{videofusion}         & 2023 & DALLE-2~\cite{dalle2}                 &  WebVid-10M~\cite{webvid}                                                                  &   \begin{tabular}[c]{@{}l@{}}VideoFusion decomposes the diffusion process by adding base noise shared by all frames  and \\ residual noise for motion along the time axis for consistent video generation.    \end{tabular}                                                                                         \\ 
Latent-Shift~\cite{latentshift}          & 2023 & LDM~\cite{stablediffusion}                 &   WebVid-10M~\cite{webvid}                                                                 & Latent-Shift adopts a parameter-free temporal modeling and reduces the training cost.                                                                                           \\ 
Video LDM~\cite{videoLDM}         & 2023 &  LDM~\cite{stablediffusion}                &  WebVid-10M~\cite{webvid}                                                                  &Video LDM has the capability to synthesize high-resolution driving scene videos lasting several minutes.
                                                                                   \\ 
PYoCo~\cite{pyoco}          & 2023 & eDiff-I~\cite{e-diff}                 &  22.5M*                                                                 & PYoCo employs progressive noise priors instead of image noise priors to train a T2V model.
         \\ 
VideoFactory~\cite{videofactory}          & 2023 &  LDM~\cite{stablediffusion}                 &   \begin{tabular}[c]{@{}l@{}}HD-VG-130M~\cite{videofactory}+\\ WebVid-10M~\cite{webvid}\end{tabular}                                                                  & VideoFactory constructs a large-scale high-definition open-domain video-text dataset, HD-VG-130M.
                                                                                          \\ 
InternVid~\cite{wang2023internvid}          & 2023 & LDM~\cite{stablediffusion}                 &   \begin{tabular}[c]{@{}l@{}}Internvid-18M~\cite{wang2023internvid}+\\ WebVid-10M~\cite{webvid}\end{tabular}                                                                  & InternVid releases an open-source 10M video-text dataset, annotated by large language models.
                 \\ 
ED-T2V~\cite{edt2v}          & 2022 &  LDM~\cite{stablediffusion}                & WebVid-10M~\cite{webvid}                                                                  & ED-T2V employs Identity attention and temporal cross-attention with low training cost for the T2V task.
   \\ 

SimDA~\cite{SimDA}          & 2023 &   LDM~\cite{stablediffusion}               & WebVid-10M~\cite{webvid}                                                                   &  SimDA designs temporal and spatial adapters for parameter-efficient fine-tuning T2V models.                                                                                         \\ 
ModelScope~\cite{modelscope}          & 2023 &   LDM~\cite{stablediffusion}               & WebVid-10M~\cite{webvid}                                                                   & ModelScope open-sources the code for T2V and serves as an important comparative baseline.    \\ 
Dysen-VDM~\cite{Dysen-VDM}          & 2023 &   LDM~\cite{stablediffusion}               & WebVid-10M~\cite{webvid}                                                                   &With the assistance of ChatGPT, Dysen-VDM can generate high-quality videos in complex action scenery.   \\ 
VideoGEN~\cite{videogen}          & 2023 &   LDM~\cite{stablediffusion}               & WebVid-10M~\cite{webvid}           &VideoGen first generates an reference image, and then combines the  image with text to generate videos.    \\ 
DSDN~\cite{videogen}          & 2023 &   LDM~\cite{stablediffusion}               &  \begin{tabular}[c]{@{}l@{}}HD-VG-130M~\cite{videofactory}+\\ WebVid-5M~\cite{webvid}\end{tabular}                                                                     & The dual-stream diffusion net could generate  amazing continuous videos with fewer flickers.  \\ 
VidRD~\cite{VidRD}          & 2023 &   LDM~\cite{stablediffusion}               &  \begin{tabular}[c]{@{}l@{}}Kinetics~\cite{kinetic}+\\ WebVid-2M~\cite{webvid}\end{tabular}                                                                     & VidRD proposes a Reused and Diffuse framework which could generate videos following the previous frames.  \\ 
LAVIE~\cite{lavie}          & 2023 &   LDM~\cite{stablediffusion}               &  20M*                                                                 & LAVIE collects high-definition videos and designs a cascaded diffusion model to generate high-resolution videos.  \\ 
Show-1~\cite{lavie}          & 2023 &   \begin{tabular}[c]{@{}c@{}}LDM~\cite{stablediffusion}+\\ DeepFloyd~\cite{deepfloyd}\end{tabular}               &  Webvid-10M~\cite{webvid}  & Show-1 is the first exploration of a video generation model that combines pixel-level and latent-level techniques.  \\ 
VideoDirGPT~\cite{videodirectorgpt}          & 2023 &   LDM~\cite{stablediffusion}              &  Webvid-10M~\cite{webvid}  & VideoDirGPT could achieve more controllable video generation by converting text into layouts.  \\ 
\bottomrule
\end{tabular}
}
\caption{Representative works summarizing and comparison in Sec~\ref{Sec:generalT2V}. We list the published year, backbone, training data and highlighted features for comparison. 
The training dataset marked "*" represents either private or newly collected datasets.}
\end{table*}




==> tex/tab_vg.tex <==
\begin{table*}[]
\centering
\scalebox{0.80}{
\begin{tabular}{@{}rllll@{}}
\toprule
Method & Year & Datasets                        & Task    & Highlight                                                                                                           \\ \midrule
VIDM~\cite{VIDM}   & 2022 & \cite{ucf101,taichi-hd, time-lapse, clevrer} & UG, CG  & VIDM synergistically combines the content generator and motion generator streams to generate videos.                 \\
GD-VDM~\cite{gd-vdm} & 2023 & \cite{cordts2016cityscapes, sun3d}               & UG, V2V & GD-VDM first generates depth videos and utilizes the depth maps to generate realistic scene videos. \\
PVDM~\cite{PVDM}   & 2023 & \cite{ucf101, time-lapse}        & UG, VP  & PVDM is one of the first latent diffusion model for video synthesis, which reduces training cost.                   \\
VDT~\cite{vdt}       & 2023      & \cite{ucf101,cordts2016cityscapes,Physion}           & UG, VP         &VDT is the first work to explore a video diffusion model based on the Transformer architecture.   \\
LaMD~\cite{lamd}       & 2023      & \cite{BAIR, time-lapse, CATER-GENs}           & VP, I2V         &LaMD is dedicated to expressing motion, thus enabling the generation of high-quality perceptual videos.\\
Generative Dynamics~\cite{generativeDynamics}       & 2023      & \cite{generativeDynamics}           & I2V         &It allows users to interact with objects in still photos and transform them into dynamic videos.\\
Video Adapter~\cite{videoAdapter}       & 2023      &  \cite{bridgedata,interactivelanguage, ego4d}                               & T2V, V2V        &  Video-Adapter explores the adaptation of general T2V models to small-scale domain-specific T2V tasks.      \\
% Animate-A-Story~\cite{Animate-A-Story} & 2023     &  \cite{webvid,ucf101}                              & T2V         &  Animate-A-Story first proposes a novel retrieval-augmented method for personalized T2V generation. \\
% AnimateDiff~\cite{AnimateDiff}   & 2023      &  \cite{webvid,huggingface, Civitai}                                & T2V        & AnimateDiff animates the personalized T2I models in a single attempt,  eliminating model-specific tuning.  \\
LEO~\cite{LEO}       & 2023      & \cite{taichi-hd,celebv, faceforensics}                                & UG,CG,VP        & LEO propose a new way for appearance and motion separation for human video generation.                                                                                                                    \\
Disco~\cite{DisCo}       & 2023     & \cite{tiktok, laion400m, deepfashion2, coco, SHHQ}                               & CG        &  Disco first establishes a novel problem setting that is referring human dance generation.                                                                                                                   \\ 
Text2Performer~\cite{Text2Performer}       & 2023     & \cite{dwnet}                               & T2V,CG        &  Text2Performer generates high-quality human videos with diverse appearances and flexible motions.                                                                                                                \\ 
LFDM~\cite{LFDM}       & 2023     & \cite{MUG, MHAD, NATOPS}                               & T2V,CG        &  LFDM first generates latent flow for conditional image-to-video with diffusion models.                                                                                                               \\ 
\bottomrule
\end{tabular}
}
\caption{Representative works summarization and comparison in Sec~\ref{Sec:Domain-specific}. We list the published year, training data, involved tasks , and highlighted features for comparison. "UG", "CG", "V2V", "VP", "I2V", "T2V" refers to unconditional generation, conditional generation, video-to-video, video prediction, image-to-video, text-to-video, respectively.}
\end{table*}

==> tex/tax_generation.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\tiny,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=2em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4.5em,font=\tiny,}{},
            where level=2{text width=3.1em,font=\tiny,}{},
            where level=3{text width=3.0em,font=\tiny,}{},
            [
                Video Generation (\S \ref{Sec:videogeneration}), ver
                [
                    Generation with \\ Text condition (\S \ref{Sec:generalT2V})
                    [
                        Training-based
                        [
                           VideoFactory~\cite{videofactory}{,}  PYoCo~\cite{pyoco} {,} Video LDM~\cite{videoLDM}{,} VDM~\cite{vdm}{,} LVDM~\cite{lvdm}{,}  Show-1~\cite{show1}   \\
                            Latent-shift~\cite{latentshift}{,} MagicVideo~\cite{magicvideo} {,} DSDN~\cite{DSDN}{,} VideoDirGPT~\cite{videodirectorgpt}{,}   Dysen-VDM~\cite{Dysen-VDM}
                            \\ Video Fusion~\cite{videofusion}{,} 
                             Imagen Video~\cite{ho2022imagenvideo}{,} VidRD~\cite{VidRD}{,} Make-A-Video~\cite{singer2022make}{,}  AnimateDiff~\cite{AnimateDiff} 
                             \\  
                            ModelScope~\cite{modelscope} {,}  VideoGEN~\cite{videogen}{,} SimDA~\cite{SimDA} {,}
                             LAVIE~\cite{lavie}
                            , leaf, text width=20.5em
                        ]
                    ]
                    [
                        Training-free
                        [
                            Text2video-Zero~\cite{Text2video-zero} {,} DirecT2V~\cite{DirecT2V}{,}
                            Free-Bloom~\cite{freebloom} 
                            DiffSynth~\cite{diffsynth}{,} LVD~
                            \cite{LVD}
                            , leaf, text width=19.5em
                        ]
                    ]
                ]
                [
                    Generation with \\ other conditions                  
                    \\ (\S \ref{Sec:modality-control})
                    [
                        Pose-guided
                        [
                            DreamPose~\cite{Dreampose}{,} Follow Your Pose~\cite{FollowYourPose} {,} Dancing Avatar~\cite{DancingAvatar}
                            , leaf, text width=18.5em
                        ]
                    ]
                    [
                        Motion-guided
                        [
                             MCDiff~\cite{MCDiff}{,} DragNUWA~\cite{DragNUWAFC}
                            , leaf, text width=7.5em
                        ]
                    ]
                    [
                        Sound-guided
                        [
                            Generative Disco~\cite{generativeDisco}{,} AADiff~\cite{aadiff} {,}
                            TPoS~\cite{TPoS}
                            , leaf, text width=11.5em
                        ]
                    ]
                    [
                        Image-guided
                        [
                            LaMD~\cite{lamd}{,} Generative Dynamics~\cite{generativeDynamics}
                            {,} LFDM~\cite{LFDM} \\
                            , leaf, text width=12.5em
                        ]
                    ]
                    [
                        Brain-guided
                        [
                            MinD-Video~\cite{Cinematic}
                            , leaf, text width=4em
                        ]
                    ]
                    [
                        Depth-guided
                        [
                            Make-Your-Video~\cite{Make-Your-Video}{,} Animate-A-Story~\cite{Animate-A-Story}
                            , leaf, text width=10.5em
                        ]
                    ]
                    [
                        Multi-Modal 
                        [
                            MovieFactory~\cite{zhu2023moviefactory}{,}
                            VideoComposer~\cite{videocomposer}{,} CoDi~\cite{CoDi}{,} Mm-Diffusion~\cite{mm-diffusion}{,} NExT-GPT~\cite{next-gpt}                            , leaf, text width=20.5em
                        ]
                    ]
                ]
                [
                    Domain-specific 
                    \\Generation (\S \ref{Sec:Domain-specific})
                    [
                        Unconditional \\ Generation
                        [
                            GD-VDM~\cite{gd-vdm}{,} PVDM~\cite{PVDM}{,} VIDM~\cite{VIDM}{,} VDT~\cite{vdt} \\ 
                            , leaf, text width=12.5em
                        ]
                    ]
                    [
                        Specific T2V
                        [
                            Video Adapter~\cite{videoAdapter}{,} NUWA-XL~\cite{nuwaxl}
                            , leaf, text width=8.5em
                        ]
                    ]
                    [
                        Human Video
                        [
                            LEO~\cite{LEO}{,} DisCo~\cite{DisCo}{,} Text2Performer~\cite{Text2Performer}
                            , leaf, text width=10.5em
                        ]
                    ]
                ]
                [
                    Video Completion
                    \\ (\S \ref{Sec:video-completion})
                    [
                        Enhance and \\  Restoration
                        [
                            LDMVFI~\cite{LDMVFI}{,} CaDM~\cite{CaDM}{,} VIDM~\cite{lookvidm}
                            , leaf, text width=10em
                        ]
                    ]
                    [
                        Video \\ Prediction
                        [
                            LGC-VD~\cite{LGCVD}{,} Seer~\cite{Seer}{,} MCVD~\cite{mcvd}{,} RVD~\cite{RVD} {,} RaMViD~\cite{RaMViD}{,} FDM~\cite{FDM}
                            , leaf, text width=18.5em
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of Video Generation. Key aspects of Video Generation include General T2V Generation, Domain-specific Generation, Conditional Control Generation, and Video Completion. }
    \label{taxo_of_videogeneration}




==> tex/taxonomy_data.tex <==
% \documentclass{article}


% \usepackage{url}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{color}
% \usepackage{threeparttable}
% \usepackage{booktabs}
% \usepackage{adjustbox}
% \usepackage{subfig}
% \usepackage{caption}
% \usepackage[misc]{ifsym}
% \usepackage{xcolor,colortbl}
% \usepackage{makecell}
% \usepackage{color}
% \usepackage{tikz}
% \usepackage[edges]{forest}
% \definecolor{hidden-draw}{RGB}{20,68,106}
% \definecolor{hidden-pink}{RGB}{255,245,247}
% \usepackage{amssymb}
% \usepackage{placeins}

% \begin{document}



\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\tiny,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure}
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\tiny,
            rectangle,
            draw=hidden-draw,
            rounded corners,
            align=left,
            minimum width=2em,
            edge+={darkgray, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt,
            line width=0.8pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        },
        where level=1{text width=2.6em,font=\tiny,}{},
        where level=2{text width=3.1em,font=\tiny,}{},
        [
             Data  \\ Evaluation (\S \ref{Sec:data-evaluation}), ver
                [
                    Data \\ (\S \ref{Sec:data}),
                    [
                        Caption-level
                        [
                            MSR-VTT~\cite{msrvtt}{, } WebVid~\cite{webvid}{, }InternVid~\cite{wang2023internvid}{, } \\HD-VILA-10M~\cite{hd-vila}
                            {, }HD-VG-130M~\cite{videofactory}
                            , leaf, text width=11em
                        ]
                    ]
                    [
                        Category-level
                        [
                            UCF-101~\cite{ucf101}{, } Taichi-HD~\cite{taichi-hd}{, }  Kinetics~\cite{kinetic}{,}  \\ Sky Time-lapse~\cite{time-lapse}{,} Cityscapes~\cite{cordts2016cityscapes}
                            , leaf, text width=11em
                        ]
                    ]
                ]
                [
                    Evaluation  \\ (\S \ref{Sec:Evaluation}),
                    [
                        Image-level
                        [
                            FID~\cite{fid}{, } CLIPSIM~\cite{clip}{, }
                            SSIM~\cite{SSIM}{,} PSNR~\cite{psnr}
                            , leaf, text width=12em
                        ]
                    ]
                    [
                        Video-level
                        [
                            FVD~\cite{fvd}{, } KVD~\cite{kvd}{, } IS~\cite{videoIS} {,} Frame Consistency~\cite{clip}
                            , leaf, text width=12.5em
                        ]
                    ]
                ]
            ]
        ]
    \end{forest}
    \caption{Taxonomy of Data and Evaluation. We list the commonly used datasets and evaluation metrics here.}
    \label{taxo_of_data}
% \end{figure}

% \end{document}


==> tex/taxonomy_editing.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\tiny,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\tiny,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=1em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=3.5em,font=\tiny,}{},
            where level=2{text width=3.8em,font=\tiny,}{},
            [
                Video Editing                 (\S \ref{Sec:videoediting})
                , ver
                [
                    Text-guided
                    \\ (\S \ref{Sec:text-guided-video-editing})
                    [
                        Training-based
                        [
                            GEN-1~\cite{gen1}{,} Dreamix~\cite{dreamix}{,} TCVE~\cite{TCVE} {,} Control-A-Video~\cite{Control-A-Video} {,}  MagicEdit~\cite{magicedit}{,} MagicProp~\cite{magicprop}
                            , leaf, text width=22.5em
                        ]
                    ]
                    [
                        Training-free
                        [
                            TokenFlow~\cite{geyer2023tokenflow}{,} EVE~\cite{EVE}{,} VidEdit~\cite{couairon2023videdit}{,} Rerender-A-Video~\cite{yang2023rerenderavideo}{,} InFusion~\cite{infusion}{,}
                            \\  Ground-A-Video~\cite{groundavideo}{,}   FateZero~\cite{qi2023fatezero}{,} Pix2Video~\cite{ceylan2023pix2video}{,} MeDM~\cite{MeDM}{,}  
                            \\
                            Vid2Vid-Zero~\cite{vid2vid-zero}{,}
                            ControlVideo$_\text{1}$~\cite{controlvideo}
                            , leaf, text width=18.5em
                        ]
                    ]
                    [
                        One-shot-tuned
                        [
                            SAVE~\cite{save}{,} EI$^2$~\cite{ei2}{,}StableVideo~\cite{chai2023stablevideo}{,}
                            Edit-A-Video~\cite{shin2023editavideo}{, } Tune-A-Video~\cite{tuneavideo}{,}\\ Video-P2P~\cite{liu2023videop2p}{,} ControlVideo$_\text{2}$~\cite{controlvideoone-shot}{,} Shape-aware TLVE~\cite{satlve} {,}                               SinFusion~\cite{Sinfusion}
                            , leaf, text width=19em
                        ]
                    ]
                ]
                [
                    Modality-guided
                    \\ (\S \ref{Sec:modality-guided-video-editing})
                    [
                        Instruct-guided
                        [
                           Instruct-vid2vid\cite{qin2023instructvid2vid}{,} CSD~\cite{CSD}
                            , leaf, text width=7.5em
                        ]
                    ]
                    [
                        Sound-guided
                        [
                            Soundini~\cite{lee2023soundini}{,} SDVE~\cite{sdve}
                            , leaf, text width=6.5em
                        ]
                    ]
                    [
                        Motion-guided
                        [
                            VideoControlNet~\cite{videocontrolnet}
                            , leaf, text width=5em
                        ]
                    ]
                    [
                        Multi-Modal
                        [
                            Make-A-Protagonist~\cite{zhao2023makeaprotagonist} {,} 
                             CCEdit~\cite{ccedit}
                            , leaf, text width=13.5em
                        ]
                    ]
                ]
                [
                    Domain-specific
                    \\ (\S \ref{Sec:domain-specific-video-editing})
                    [
                        Recolor\&Restyle
                        [
                            ColorDiffuser~\cite{colorDiffusers}{,} Style-A-Video~\cite{styleavideo}
                            , leaf, text width=9em
                        ]
                    ]
                    [
                        Human Video
                        [
                            Diffusion Video Autoencoders~\cite{diffusionvideoautoencoder}{,} Instruct-Video2Avatar~\cite{instruct-video2avatar}{,}  TGDM~\cite{tgdm}
                            , leaf, text width=17.5em
                        ]
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of Video Editing. Key aspects of Video Editing include General Text-guided Video Editing, Modality-guided Video Editing  and Domain-specific Video Editing. }
    \label{taxo_of_mcot}
\end{figure*}



==> tex/taxonomy_understanding.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure}[t!]
    \centering
    \resizebox{0.8\linewidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\scriptsize,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=8.0em,font=\scriptsize,}{}, 
            [
                Video Understanding (\S \ref{Sec:video-understanding})
                , ver
                [
                    Temporal Segmentation
                    % \\ (\S \ref{Sec:detection-segmentation})
                    [
                        DiffTAD~\cite{difftad}{,} DiffAct~\cite{diffact}
                        , leaf, text width=9em
                    ]
                ]
                [
                    Video Anomaly Detection
                    % \\ (\S \ref{Sec:video-anomaly-detection})
                    [
                        Diff-VAD~\cite{DiffVAD}{,} CMR~\cite{UVAD}{,} \\ MoCoDAD~\cite{MoCoDAD}
                        , leaf, text width=9em
                    ]
                ]
                [
                    Text-Video Retrieval, text width=6.5em
                    % \\ (\S \ref{Sec:text-video retrieval})
                    [
                        DiffusionRet~\cite{jin2023diffusionret}{,}  MomentDiff~\cite{momentdiff} \\ DiffusionVMR~\cite{diffusionvmr}
                        , leaf, text width=11.0em
                    ]
                ]  
                [
                    Video Captioning
                    % \\ (\S \ref{Sec:video-caption})
                    [
                         RSFD~\cite{RSFD}
                        , leaf, text width=4em
                    ]
                ]   
                [
                    Video Object Segmentation, text width=8.3em
                    % \\ (\S \ref{Sec:video-object-segmentation})
                    [
                        Pix2Seq-D~\cite{pix2seq-D}
                        , leaf, text width=5em
                    ]
                ]     
                [
                    Video Pose Estimation
                    % \\ (\S \ref{Sec:video-pose-estimation})
                    [
                        DiffPose~\cite{feng2023diffpose}
                        , leaf, text width=4.5em
                    ]
                ]  
                [
                    Audio-Video Separation
                    % \\ (\S \ref{Sec:audio-video-separation})
                    [
                        DAVIS~\cite{huang2023davis}
                        , leaf, text width=4.5em
                    ]
                ]
                [
                    Action Recognition 
                    % \\ (\S \ref{Sec:action-recognition})
                    [
                        DDA~\cite{DDA}
                        , leaf, text width=4.5em
                    ]
                ]
                [
                    Video Soundtracker 
                    % \\ (\S \ref{Sec:soundtracker})
                    [
                        LORIS~\cite{LORIS}
                        , leaf, text width=4.5em
                    ]
                ]
                [
                    Video Procedure Planning 
                    % \\ (\S \ref{Sec:soundtracker})
                    [
                        PDPP~\cite{wang2023pdpp}
                        , leaf, text width=4.5em
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of diffusion-based Video Understanding. Key aspects of Video Understanding include Temporal Action Detection, Anomaly Detection, Text-Video Retrieval, Video Captioning and Video Segmentation. }
    \label{taxo_of_lavr}
\end{figure}



